Generative Denoise Distillation: Simple Stochastic Noises Induce Efficient Knowledge Transfer for Dense Prediction

Knowledge distillation is the process of transferring knowledge from a more powerful large model (teacher) to a simpler counterpart (student). Numerous current approaches involve the student imitating the knowledge of the teacher directly. However, redundancy still exists in the learned representations through these prevalent methods, which tend to learn each spatial location's features indiscriminately. To derive a more compact representation (concept feature) from the teacher, inspired by human cognition, we suggest an innovative method, termed Generative Denoise Distillation (GDD), where stochastic noises are added to the concept feature of the student to embed them into the generated instance feature from a shallow network. Then, the generated instance feature is aligned with the knowledge of the instance from the teacher. We extensively experiment with object detection, instance segmentation, and semantic segmentation to demonstrate the versatility and effectiveness of our method. Notably, GDD achieves new state-of-the-art performance in the tasks mentioned above. We have achieved substantial improvements in semantic segmentation by enhancing PspNet and DeepLabV3, both of which are based on ResNet-18, resulting in mIoU scores of 74.67 and 77.69, respectively, surpassing their previous scores of 69.85 and 73.20 on the Cityscapes dataset of 20 categories. The source code is available at https://github.com/ZhgLiu/GDD.

==> tbl/abl.tex <==
\begin{table*}
\centering
\label{tab:scenario_generation_metrics}
\begin{tabular}{lcccccc} 
\toprule
\textbf{Model}       & \textbf{Collision (\%)} & \textbf{Off-road (\%)} & \textbf{Progress (m)} & \textbf{Wrong Direction(\%)} & \textbf{Realism} \\ 
\midrule
Ours (- $J_{gc}$)    & 30.82                   & 0.46                   & 48.1                  & \textbf{8.72}                         & 0.71                \\
Ours (- $J_{route}$)       & \textbf{3.03}                    & 3.48             & 51.2                  & 23.9                         & 1.08               \\
Ours (- clean guide) & 5.15                    & \textbf{0.32}                   & 11.8                 & 4.65                         & \textbf{0.55}                      \\
Ours                 & 4.21                    & 1.15                   & \textbf{56.8}                  & 9.37                         & 0.96                \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study on diffusion model guidance functions.} Results show the effectiveness of $J_{gc}$ in reducing collision rates, the role of $J_{route}$ in managing wrong-direction incidents, and the impact of clean guidance on improving the progress of reactive agents.}
\label{tab:abl}
\vspace{-1em}
\end{table*}


==> tbl/adv_sup.tex <==
\setlength\tabcolsep{4 pt}
\begin{table*}
% \begin{center}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Other Offroad} & \textbf{Adv Offroad} & \textbf{Coll Speed} & \textbf{Realism}  \\
                                 & (\%) $\uparrow$       & (\%) $\uparrow$         & (\%) $\downarrow$      & (\%) $\downarrow$    & (m/s) $\downarrow$  & $\downarrow$      \\ 
\midrule
Ours (- $J_{route}$)~              & 47.1                  & 50.0                    & 25.5                   & 28.0                 & \textbf{2.19}       & 0.56              \\
Ours~ (- clean guide)            & \textbf{51.2}         & \textbf{51.2}           & \textbf{14.6}          & 17.1                 & 2.20                & 0.61              \\
Ours                             & 38.2                  & 42.7                    & 23.2                   & \textbf{8.8}         & 2.63                & \textbf{0.48}     \\
\bottomrule
\end{tabular}
}
\captionof{table}{\textbf{Ablation study on diffusion model guidance functions for safety-critical simulation.}We compare the performance of our approach with and without our proposed ``route'' and ``clean'' guidance functions when generating safety-critical traffic simulations. Our guidance lead to enhanced performance in Ego-Adversary collision rate with reduced adversary's off-road rate and improved realism}
\label{tab:supp_adv}
\end{table*}

==> tbl/ctg.tex <==
\begin{table*}
\centering
\begin{tabular}{lcccccc} 
\toprule
 \multirow{2}{*}{\textbf{Method}}   & \textbf{Coll Rate} &\textbf{Off Road } &\textbf{Failure Rate} &\textbf{Wrong Direction} & \textbf{Realism} \\ 
   & (\%) $\downarrow$ & (\%) $\downarrow$ & (\%) $\downarrow$ & (\%) $\downarrow$ & $\downarrow$ \\ 
\midrule
CTG no collision & 4.0  & 27.1   & 27.1                                                                          & -                                                                                          & \textbf{0.569}           \\
CTG off-road     & 11.4                                                                       & 34.1                                                                      & 45.5                                                                          & -                                                                                          & \textbf{0.569}           \\
CTG*~            & 21.84                                                                      &\textbf{ 0.13}                                                                      & 21.96                                                                         & 9.31                                                                                       & 0.754           \\
Ours             & \textbf{3.49}                                                                       & 0.87                                                                      & \textbf{4.18}                                                                          & \textbf{6.54}                                                                                       & 0.87                      \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparative Analysis in Closed-Loop Traffic Simulation.}  While our approach exhibits a slightly higher realism, it significantly outperforms both CTG versions in terms of reduced failure rate and improved wrong direction rate, highlighting the efficacy of our proposed guidance strategies.}

\label{tab:ctg}
\vspace{-1em}
\end{table*}

==> tbl/ctrl_ttc.tex <==
\begin{table*}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{cc|ccc|cc} 
\toprule
% \multicolumn{1}{l}{}           & \multicolumn{4}{c}{\textbf{Metric}}            \\ 
% \midrule
 \multirow{2}{*}{\textbf{TTC Cost weight}} & \multirow{2}{*}{\textbf{TTC Cost}}  & \textbf{TTC} &\textbf{Coll Speed} & \textbf{Coll Angle} & \textbf{Coll Rate} & \textbf{Realism}  \\ 
&  & (s) & (m/s) & (deg) & (\%) $\uparrow$ & $\downarrow$  \\ 
\midrule
0.0                   & 0.24     & 11.39   & 2.45 & 12.76 & 0.53           & 0.83     \\
1.0          & 0.29     & 6.83    & 2.30 & 6.47 & 0.50           & 0.89     \\
2.0                   & 0.36     & 3.03    & 3.78 & 1.00 & 0.7            & 0.88     \\
\bottomrule
\end{tabular}
\caption{\textbf{Evaluating Time to Collision (TTC) Control.} The table shows the impact of different TTC Cost weights on collision scenarios. Increasing the TTC Cost weight results in a decrease in time to collision and an increase in collision rate, suggesting a heightened challenge for the ego vehicle in avoiding collisions.}
% }
\label{tab:ctrl_ttc}
\vspace{-1em}
\end{table*}
% THBD\\




==> tbl/ctrl_v.tex <==
\begin{table}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|cc}
\toprule
 {\textbf{Rel Speed}} & \textbf{Ego-Adv Rel} & \textbf{Coll Rate} & \textbf{Realism}  \\ 
  \textbf{Control} (m/s) & \textbf{Speed} (m/s) & (\%) $\uparrow$ & $\downarrow$ \\ 
\midrule
-2.0                               & 0.90                    & 0.38           & 0.83              \\
0.0                       & 1.26                    & 0.38           & 0.89              \\
2.0                                & 1.94                    & 0.50           & 0.88              \\ 
\midrule
No control                                  & 3.94                    & 0.72           & 0.82             \\
\bottomrule
\end{tabular}
\caption{\textbf{Controllability of relative collision speed.} This table illustrates the ability of our framework to modulate the relative speed between ego and adversarial agents, influencing collision rates while maintaining realism.}
% }
\label{tab:ctrl_v}
\end{table}


==> tbl/ddim_abl_sup.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\centering
\caption{\textbf{Ablation Study on Accelerated Sampling through Different DDIM Steps.} The table illustrates a performance degradation with fewer diffusion steps. Notably, DDIM with 10 steps still maintains a relatively low failure rate.}
\label{tab:ddim}
\begin{tabular}{lcccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Coll Rate} & \textbf{Off Road} & \textbf{Failure Rate} & \textbf{Wrong Direction} & \textbf{Progress} & \textbf{Realism}  \\
                                 & (\%) $\downarrow$  & (\%) $\downarrow$  & (\%) $\downarrow$     & (\%) $\downarrow$        & (m) $\uparrow$    & $\downarrow$      \\ 
\midrule
DDIM (10 steps)                  & 3.58               & 5.34               & 8.78                  & 16.97                    & \textbf{65.4}     & 0.93              \\
DDIM (5 steps)                   & 3.79               & 9.53               & 12.84                 & 20.71                    & 62.4              & 0.83              \\
DDIM (1 step)                    & 3.47               & 11.16              & 14.03                 & 21.41                    & 58.9              & \textbf{0.53}     \\
DDPM (100 steps)                 & \textbf{1.74}      & \textbf{4.40}               & \textbf{6.05}         & \textbf{9.73}            & 51.3              & 0.88              \\
\bottomrule
\end{tabular}
\end{table*}


==> tbl/diff_planner_sup.tex <==
\begin{table*}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} 
\toprule
\multicolumn{1}{c|}{\textbf{Planner}} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Adv Offroad} & \textbf{Coll Speed} & \textbf{Ego Accel } & \textbf{Realism}  \\
                                  & (\%) $\uparrow$       & (\%) $\uparrow$         & (\%) $\downarrow$    & (m/s) $\downarrow$  & (m/s\(^2\)) $\downarrow$             & $\downarrow$      \\ 
\midrule
BC                                & 40.3                  & 43.3                    & 20.9                 & 2.65                & 0.60                                   & 0.83              \\
IDM                               & \textbf{49.3}         & \textbf{58.2}           & 15.0                 & \textbf{-0.37}      & 1.09                                   & 0.85              \\
Lane-graph                        & 35.8                  & 38.8                    & \textbf{13.4}        & 2.34                & 2.51                                   & \textbf{0.60}     \\
\bottomrule
\end{tabular}
% }
\captionof{table}{\textbf{Safety-Critical Simulation for different Planner settings}}
\label{tab:supp_diffplan}
\end{table*}


==> tbl/strive.tex <==
\setlength\tabcolsep{4 pt}

\begin{table*}[!ht]
\centering

% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|cccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Length} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Other Offroad} & \textbf{Adv Offroad} & \textbf{Adv Speed} & \textbf{Realism}  \\
& (s)  & (\%) $\uparrow$  & (\%) $\uparrow$  & (\%) $\downarrow$ & (\%) $\downarrow$  &  (m/s) $\downarrow$ &  $\downarrow$            \\
\midrule
STRIVE   & 6    & 36.7   & 38.2  &  \textbf{16.1}  & 25.0 & 4.01 & 0.85              \\
Ours     & 6    & 25.0   & 26.5  & 18.0 & 11.8 & \textbf{2.04} & \textbf{0.43}              \\
Ours     & 12   & \textbf{38.2}  & \textbf{42.7}  & 23.2  & \textbf{8.8}  & 2.63 & 0.48              \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison between STRIVE \cite{strive} and our approach for safety-critical generation for a rule-based planner.}. Our framework demonstrates enhanced performance in Ego-Adversary collision rate with reduced adversary's off-road rate and improved realism}
% }
\label{tab:strive}

\end{table*}
\setlength\tabcolsep{6 pt}
